Unsupervised Sound Localization via Iterative Contrastive Learning

Sound localization aims to find the source of the audio signal in the visual scene. However, it is labor-intensive to annotate the correlations between the signals sampled from the audio and visual modalities, thus making it difficult to supervise the learning of a machine for this task. In this work, we propose an iterative contrastive learning framework that requires no data annotations. At each iteration, the proposed method takes the 1) localization results in images predicted in the previous iteration, and 2) semantic relationships inferred from the audio signals as the pseudo-labels. We then use the pseudo-labels to learn the correlation between the visual and audio signals sampled from the same video (intra-frame sampling) as well as the association between those extracted across videos (inter-frame relation). Our iterative strategy gradually encourages the localization of the sounding objects and reduces the correlation between the non-sounding regions and the reference audio. Quantitative and qualitative experimental results demonstrate that the proposed framework performs favorably against existing unsupervised and weakly-supervised methods on the sound localization task.

==> backup/1_intro_bk.tex <==
\section{Introduction}\label{sec:intro}

% \yb{To describe problem and the importance of this topic. (e.g, the sound localization would benefit downstream audio-visual tasks like av separation. Since ...) or refer to other CVPR/ECCV paper.}\\

% 1. the goal of the sound localization tasks
% 2. why does this problem important? describe some down-stream applications
Multisensory signals (\eg vision, touching, and hearing) provide rich information when human beings perceive the environment.
%When human beings perceive the environment, the multisensory signals (\eg vision, touching, and hearing) provide rich information.  
%When human beings perceive multisensory feelings in the world (e.g., vision, touching, and hearing), the data from different modalities provide rich information, which enable human beings to achieve complicated tasks in our daily life. 
%
Moreover, these different modalities are usually intertwined and thus enable human beings to achieve complicated tasks in our daily lives.
%
Take audio and vision as example, we can easily imagine a lightning scene upon hearing thunders, we can associate multiple objects with their sources on a noisy street, and we can easily identify and converse with our friends in a crowded cocktail party. 
%
In this work, we target at the \emph{sound localization} task ~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_mms_loc,av_nips20_loc} which aims to find regions co-occurring with audio events.
% \james{the definition looks weird to me}
%Take audio and visual as example, human beings are able to do tasks including recognizing objects, separating clear from mixed signal, localizing sound, etc. In this work, we will target at \textit{sound localization} ~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_mms_loc,av_nips20_loc}, which requires one to identify objects and determine whether objects make sound or not \ybTodo{(in Fig??)}. 
% 
The sound localization algorithms serve as the cornerstone techniques to various audio-visual applications such as audio-visual source separation~\cite{pix,av_eccv18_sep,co_sep_iccv19,sofm_iccv19,av_iccv19_mpnet,av_cvpr20_sep-gesture} and audio-visual event localization~\cite{eccv18_avel,av_eccv20_avvp}.
%A good sound localization algorithm can serve as a cornerstone to various audio-visual applications such as audio-visual source separation and audio-visual event localization.
% \ybc{need citation or not ?}\hyt{yes}
% \james{One more use case here.}
%Therefore, it would be desirable if one can design a machine to identify the sounding regions of interest in a scene, which is a stepping stone to understand multisensory data in the world. 
%
%The capability of sound localization can benefit audio-visual tasks such as audio-visual source separation~\cite{co_sep_iccv19, pix,sofm_iccv19} because it requires the model to identify sounding objects and separate their sound. 
% \james{kinda weird to narrow down so fast "we can achieve complicated tasks!!"->"btw, sound localization is rly great". Might be better: human can handle multiple sensor joinly->take audio/visual as example, human can do tasks including...->in this work, we'll target at localization, which is ....}



% \yb{To tackle with this problem. some work.... how to deal with this problem.} \hyt{describe the challenges of this task first, then summarize the current solutions and their drawbacks in next paragraph.}\\

% challenges in this tasks:
% 1. lack of audio/image source localization annotation (e.g., bounding box) 
% 2. the sound source may come from partial region of an image
% 3. ...
\input{figure/teaser}
% \hyt{need to revise the flow of this paragraph, see comments in the slack}
Sound localization approaches based on deep learning require a large amount of training data with the annotations of sound-visual association.
% Since associating sound and objects requires supervision from jointly observing both audio and visual data, the annotations of sounding regions is difficult to access.
%
% \james{still, it is not "difficult for a machine", it's difficult for human to label. So, assume we have perfect data, we can train perfect models? If not, we can say: "Data is a big issue cuz label is hard to get->someone propose dataset->however, even with perfect data, the leraning is still not easy because XYZ"}
% \james{I cannot get it why this is an issue}
%
To this end, Senocak~\etal~\cite{av_cvpr18_lls,av_tpami20_lls} propose the first sound localization dataset containing bounding box annotations of sounding regions.
% and a sound localization framework \hyt{not necessary to have "a sound localization framework" as it is never mentioned hereafter"}.
%
These annotations provide the supervised guidance for models to learn from audio/visual information.
%semi-supervised and unsupervised manner.
%\james{why mention semi and unsupervised here???}
%\ybc{20,21 did not present fully supervised results}
% \james{How does this dataset resolve the difficulty above? or they are two different issues (data and partial regions?)}
% 
Nevertheless, the annotated images with sounding regions are not sufficient (only 5k annotations). 
%
We note that, it is arduous to collect a large amount of sounding regions annotations due to the labor-intensive annotation process, which requires annotator to jointly observe visual and audio signals and easily results in noisy data.
% Nevertheless, even with annotations data, by observing audio and visual inputs to localize sound is still a challenging task because complex scenes only provide imprecise sounding region information to associate corresponding sound.
% 
%Several methods~\cite{av_cvpr18_lls,av_tpami20_lls,av_arxiv_curricumlum_av_clutser,av_cvpr19_deep_cluster} tackle with that issue by leveraging the image-audio correspondence information to achieve sound localization in a (semi-) unsupervised manner.
% Several efforts have been made to learn the sound localization task.
% 
%Nevertheless, merely using the audio-visual correspondence is not informative enough since the image may contain non-sounding or ambient regions, which would associate incorrect sounding object and audio signals.

% \yb{However, the drawback of these methods and limitation.}\hyt{summarize current solutions and their drawbacks here}\\
To tackle the task with limited data, several methods are proposed in a weakly supervised manner with audio-visual event labels~\cite{av_eccv20_mms_loc} or a self-supervised manner by leverage image-audio correspondences~\cite{av_cvpr18_lls,av_tpami20_lls} and audiovisual clusters~\cite{av_arxiv_curricumlum_av_clutser,av_cvpr19_deep_cluster}.
%
%methods~\cite{av_cvpr18_lls,av_tpami20_lls,av_arxiv_curricumlum_av_clutser,av_cvpr19_deep_cluster} tackle issue by leveraging the image-audio correspondence information to achieve sound localization in a (semi-) unsupervised manner
%Without any supervision of sounding regions, a number of methods~\cite{av_eccv20_mms_loc,av_arxiv_curricumlum_av_clutser,av_cvpr19_deep_cluster} jointly leverage audio-visual representations have been proposed.
% \hyt{consider "feature" is confusing, just say leverage audio-visual feature representation learning}
% \ybc{w/o location annotation. audio/visual events are weaker supervision than location one}
% \james{What does it mean by "prior knowledge on sounding regions"? labelled audio/visual events seem to be a strong human prior annotation to me}
%
%Audiovisual clusters~\cite{av_cvpr19_deep_cluster,av_arxiv_curricumlum_av_clutser} are built up to associate audio signal and visual regions, and Qian~\etal~\cite{av_eccv20_mms_loc} exploit audio/visual event labels to find out potential sound regions. 
%
However, all these methods rely on certain extent of human prior knowledge such as the pre-defined number of clusters~\cite{av_cvpr19_deep_cluster,av_arxiv_curricumlum_av_clutser} or image-level audio-visual event labels~\cite{av_eccv20_mms_loc}.
%
Furthermore, using the audio-visual correspondence alone is not informative enough since the image may contain non-sounding or ambient regions, which will lead to the association between incorrect sounding object and audio signals.
%
These constraints limit the generalization of sound localization in unconstrained scenarios (e.g., single/multiple sound sources, objects undefined in the annotations).
%\james{still not sure what you mean novel. Is it unseen objects during training?}
%\ybc{Some objects may not be defined in label spaces. }
% \james{"unseen" is ambiguous, it can refer to unseen instances during training, occluded objects in a scene, background sound, etc}
%
% \james{quite wordy, can move most of these to related work. Might be better to state sthg like: There are n branches of work -> But they require either A~\cite{}, B~\cite{}, or C~\cite{}. -> They are bad bad.}
% \yb{To address aforementioned issue. We exploit ... and ... to ...., which can further ??? to benefit av-localization task. (high level) }\\

% In this paper, we propose .....
% Contribution 1: briefly introduction -> address what challenges listed in paragraph #2 (e.g., we propose a iterative contrastive learning algorithm -> address the lack of audio/image source localization issue)
% contribution 2: ....
% contribution 3: ....
% yb: iterative ->  decompose visual objects
%  inter -> associate event w/o supervision and false negative?
%  intra -> exclude non-interest objects w/o labels
%In this work, we propose an iterative contrastive representation learning algorithm without any prior assumption or event label for the sound localization task.
In this work, we propose an iterative contrastive representation learning algorithm which does not require any prior assumption or event labels.
% to address the issue of lacking annotations.
% To accurately associate sounding objects and sound, we propose an iterative contrastive learning algorithm, which includes potential sounding regions and exclude non-interest objects without any prior assumption/event labels.
% \hyt{"includes potential sounding regions and exclude non-interest objects" is what sound localization does. $\rightarrow$ In this work, we propose an iterative contrastive representation learning algorithm without the requirement of prior assumption/event labels for the sound localization task.}
% \james{so...this sentence indicates that the major goal and main features for the proposed method is to "eliminate sielent objects"???}
%
We illustrate the core idea of our method in \figref{teaser}.
%
Starting from the conventional contrastive learning (\textit{baseline} in \figref{teaser})~\cite{av_iccv17_look,av_eccv18_obj_that_sound,av_nips16_soundnet,av_eccv16_abSound} \ybc{put the ref. in audio-visual learning with baseline sampling technique}
% \hyt{(should we have a citation for infoNEC here?)}
, the proposed approach uses the sound localization model obtained in \emph{previous} epoch to estimate sounding and non-sounding regions as the \emph{pseudo}-labels for the current training epoch.
%To be more specific, the core idea is to utilize the sound localization trained in \emph{previous} epoch to sample the (non-)interest regions to be considered in the current training epoch.
% Specifically, sounding regions of (non-)interest from previous(?) model are considered during current model training.
% \hyt{basically you want to describe what "iterative" is for $\rightarrow$ The core idea is to use the sound localization model trained in the \emph{previous} epoch to sample the (non-)interest regions to be considered in the current training epoch.}
%
% Since there are a few objects making sound in visual scenes, audio signal would be a favorable guidance to model the correlation of audio-visual data. \james{cannot understand this}
%
In addition to exploiting the relations between audio and visual signals within an instance, we further leverage the relationships among audio signals across instances, as the \emph{inter-frame relation} shown in \figref{teaser}.
%Furthermore, we leverage the relationship between audio signals to guide the audio-visual learning.
%
\yb{Specifically, the representations of different sounding objects should be similar if the corresponding audio instances are highly correlated, which preventing pulling sounding objects away from related audio signals with naive contrastive learning.
%HYT
%when audio instances are highly correlated, it indicates that the corresponding sounding objects are likely to be similar.
%
It would be a reliable guidance to learn accurate sound localization by exploring relationship between audio instances.}
%\james{Why? Is it: prevent sounding obj not ass with related audio signgla, or prevent audios signal ass with unrelated sounding obj??}
%\ybc{The former one is correct. e.g., if two pairs contain train in it, but original one would repel the distance between these pairs.} % 避免應該要拉近的 卻被推遠
% Furthermore, in order to preserve the relationship between audio and visual data without any supervision,
% we exploit the correlation between all the audio instances to model the relationship in audio-visual data. 
% %
% In other words, the relationship between audio-visual and audio data should be consistent. 
% %
% Such correlation information would guide our model to associate the same event audio signal and objects even lacking of labels supervision. 
% \hyt{see the comment in the slack}
%
We evaluate the proposed method on the SoundNet Flickr dataset~\cite{av_cvpr18_lls,av_tpami20_lls} with the consensus intersection over union (cIoU) and area under curve (AUC) as evaluation metrics.% to support the effectiveness of our framework.
%
Both the qualitative and quantitative results demonstrate the effectiveness of the proposed method. 
% \james{Quite vague, I cannot tell what exactly we propose at the first glance. Might do: We propose an awesome algo-> First, to handle X, we use \textbf{XX}. Second, to handle Y, we use \textbf{YY}}
% \james{Experiments missing. Just need to mention, we use XYZ metrics on ZYX datasets. We beat them all. We good}

% \hyt{[optional] briefly describe the experiments}\\
% \yb{To highlight our key contribution..}\\
%%%%%%%%%%%%%%%%
The contributions of this paper are highlighted below:
\begin{compactitem}
  \item We propose an iterative contrastive learning algorithm for the unsupervised sound localization task without the requirement of data annotations. %HYT
  %We propose a unsupervised training strategy for the sound localization task.
  %
  %The proposed iterative contrastive learning algorithm can associate audio signals to regions of interest.
  %which excludes non-interest regions for robust training, which prevents non-sounding objects associated with audio source.
  %
  \item We propose to leverage not only the regions of interests, but also exploit the non-sounding regions and the relationship across audio instances to jointly learn the audio and visual representations.
  %\ybc{may sounding regions of non-interest be confusing? means non-sounding?}
  %which guides the sound localization process with improved performances.
  %
  \item Qualitative and quantitative experiments on the benchmark dataset demonstrate that the proposed method performs favorably against state-of-the-art \emph{weakly supervised} and \emph{unsupervised} approaches. %with any  and confirm that the learning scheme can be deployed without any human supervision.
%   
  %\james{Btw, isn't our results are way better than the weakly-supervised method? Should stress it somewhere}
\end{compactitem}



==> backup/2_related_bk.tex <==
\section{Related Work}
\Paragraph{Self-Supervised Audio-Visual Representation Learning.} 
%
%Videos provide natural supervision via inherent correlation among modalities, which serve as natural supervisory signal for training a model.
The inherent correlation among different modalities of a video provides natural supervisory signals for learning a deep neural network model.
%provides vital information to train a machine to understand it without human supervision. 
%
Existing self-supervised audio-visual representation learning methods
can be broadly categorized as follows. 
% simple supervision
First, audio-visual pairs are extracted from a video clip as positive correlation. 
%
The assumption is that the audio and visual features should be strongly correlated if they are extracted from the same video clip~\cite{av_iccv17_look,av_eccv18_obj_that_sound,av_nips16_soundnet,av_eccv16_abSound}. 
%
%When audio and visual features are extracted from the same video clip, the audio and visual representation should be highly correlated. 
%The audio and visual features should be correlated if they are extracted from the same video clip.
%
In addition, these schemes differentiate the features extracted from the unpaired video clips.
%assume the correlation between unpaired audio and videos should be low.
% \james{"respectively" implies you mean correlation between audios from different videos should be low, so do videos. But it should be unpaired videos and audios have low correlation}
Furthermore, some approaches~\cite{av_arxiv_agreement,avt_nips20_VersatileNet} consider the correlation within each modality or across more modalities (i.e., audio, vision, and text) to optimize models.
%\james{can not quite get it what is the correlation in a single modality}
%\ybc{should be "each": correlation in audio/visual modality respectively [16]}
% 
Second, temporal information with a video is considered to determine strong or weak correlation. 
%
%MH: check this sentence
%A few methods sample audio and visual features extracted from the same video as strong correlation, and consider those across different time instances as weak correlation for the representation learning~\cite{av_eccv18_Owens,av_nips18_coop}.
Given a video sequences, a few methods sample the audio and visual features extracted from the same time frame as strong correlation, and consider those across different time instances as weak correlation for the representation.
%
Third, spatial relations among image regions are exploited. 
%jointly modeling spatial audio and vision: 
%
Since the binaural recording techniques (spatial audio) preserve the spatial information of the sound origins, some approaches~\cite{av_nips20_spatial_alignment,av_eccv20_sep-stereo,av_cvpr20_tell_left_right,25d,360gen} jointly model the visual and audio information spatially to construct spatial audio generation systems or learn representations for downstream tasks.
%associate visual and audio information, especially binaural recording to build spatial audio generation systems or deploy on downstream tasks. 
%


%However, we note that, the mainstream media contain only monaural recording (single channel). Therefore, we mainly focus on monaural audio localization in visual scenes.
%In this work, we focus on monaural audio localization in visual scenes.
%
%Even though the aforementioned methods present decent results on video-based applications, only the relationship of audio-visual pairs across videos or time but same videos is considered during learning process.
%
%We propose a framework, which benefit from further exploring the relationship between objects in the same visual scenes and audio signal across pairs, to learn discriminative audio-visual features on sound localization task.
% \james{kinda weird to spend quite a lot of words on spatial audio}
% \james{It's quite unorganized. Maybe I'll organize them this way: Videos provides natural supervision via inherent correlation among modalities. There are three branches. First, audio-visual pair. Second, taking temporal into consideration. Third, taking spatial into consideration.}
\input{figure/fig_method}
\Paragraph{Sound Source Localization in Visual Scenes.}
Sound source localization in visual scenes aims to find sounding regions from audio signals. 
%
We summarize the methods for tackling this problem into three categories.
% Recently, some works~\cite{av_eccv18_obj_that_sound,av_eccv18_Owens,eccv18_avel} either utilize the correspondence between audio and visual patches or class activation map (CAM)~\cite{cvpr16_CAM} to explore sounding regions.
%
%First, the correspondence between audio and visual signal provides guidance to training~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_objs_vids}.
The first group of work~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_objs_vids} leverages the correspondence between audio and visual signals for supervision.
%
The assumption is that the audio and visual features extracted from the same video clip should be similar, while those extracted from different clips are differentiated.
%the aaaudio-visual correspondence learning: by exploiting audio and visual features from video clips, audio /visual features should be similar from the same video clips. 
%
%Otherwise, audio-visual representations from the different video clips are likely to be dissimilar.  
%
%some works~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_objs_vids} are proposed with this kind of guidance. 
%
Some sound localization methods~\cite{av_cvpr18_lls,av_tpami20_lls} are formulated within the semi-supervised framework to deal with limited annotated data.
%
%train the models in a semi-supervised fashion, which utilize sounding regions annotations.
%
%Since it is arduous to collect the annotations of sounding regions due to the labor-intensive
%annotation process, methods without these annotations would be valuable.
%Second, class activation map (CAM)~\cite{cvpr16_CAM}-based methods are proposed without the annotation of sounding regions.
%CAM can interpret the prediction decision made by models and indicate discriminative regions used for categorical prediction.
The second line of work uses the class activation map (CAM)~\cite{cvpr16_CAM} to determine discriminative regions used for categorical prediction.
%
%Since CAM is able to explore salient image regions by classes, 
Owens \etal~\cite{av_eccv18_Owens} learn the audio and visual representations by the audio-visual correspondence and perform sound localization using the CAM model. 
% 
%Similarly, in~\cite{av_eccv20_mms_loc}, given audio/visual event labels, audio signal and regions of corresponding events are extracted by CAM 
Similarly, given the event labels, Qian \etal~\cite{av_eccv20_mms_loc} use the CAM model to extract sounding regions and corresponding audio clips.
%
As such, the sound and visual object in the same event can be associated.
%
Finally, some models~\cite{av_cvpr19_deep_cluster,av_arxiv_curricumlum_av_clutser} utilize audio-visual clusters to model audio-visual relationships.
%
These methods cluster different frequencies of audio signal and visual patches in the images.
%
The centered features of the audio and visual clusters extracted from the same video clip are associated during the training stage.


We note that existing sound localization approaches are limited in several aspects. 
%
These methods typically require additional information in other modality (\eg optical flow~\cite{av_eccv20_objs_vids}), pre-defined number of sound source~\cite{av_cvpr19_deep_cluster,av_arxiv_curricumlum_av_clutser}, event labels in both audio and visual modalities~\cite{av_eccv20_mms_loc}, or single-source videos~\cite{av_nips20_loc}. 
%
In this work, we present a sound localization framework without the requirement of any annotation or assumption. 
%
Furthermore, the correlation between (non-)sounding objects and audio across pairs are jointly considered in our model to localize sound sources accurately. 
% \james{Similar to the previous paragraphs, it's quite unorganized. Do not just list works out like A does X, B does Y, C..... But try to cluster them in high-level concept.}

% \yb{Audio-Visual Separation???} 
% \hyt{have this only if we have the separation results in the exp.}


==> backup/3_method_bk.tex <==

\section{Methodology}
\label{sec:method}

\subsection{Preliminaries}
Our goal is to learn a sound localization model in an unsupervised fashion.
%
During the testing time, we are given the input image of shape $W\times H\times 3$ and the detected audio (\ie sound).
%
We denote the term $M=WH$.
%
As shown in the top side of \figref{method}, the proposed sound localization model first extracts the corresponding visual representation $\mathbf{V}=[\mathbf{v}_1,\cdots,\mathbf{v}_M]\in\mathbb{R}^{M \times d}$ and audio feature $\mathbf{a}\in\mathbb{R}^{1 \times d}$ from the input image and the short-time Fourier-transformed~\cite{stft} audio, respectively.
%
To localize the sounding source in the image, we use the attention mechanism to compute the response map $\mathbf{R}=[\mathbf{r}_1,\cdots,\mathbf{r}_M]\in\mathbb{R}^{M\times 1}$, where
\begin{equation}
    \mathbf{r}_i = \mathbf{v}_i^\top \cdot \mathbf{a}\hspace{5mm} i = 1,\cdots,M.
\end{equation}
%
Then the sounding region $\mathbf{S}\in\mathbb{R}^{w\times h\times 3}$ is determined by thresholding the response map $\mathbf{R}$.


In Section~\ref{sec:av-learning}, we first introduce the initial audio-visual training scheme with contrastive learning as the paradigm for the following epochs. 
% 
We then further present our iterative learning strategy and proposed sampling techniques to learn discriminative audio-visual features. 
% 
How sound localization task can be achieved by audio-visual response will be demonstrated in section~\ref{sec:results}.


% \hyt{Use the notation to describe the problem to be solved (can refer to the method overview figure)}
% We first define the notations and settings for sound localization in this paper. 
% problem
Our goal is to associate sounding regions $\mathbf{v}\footnote{note that $w,h$ is smaller compared with original image inputs for simplicity} \in \mathbb{R}^{d \times w \times h}$ and corresponding audio signal $\mathbf{a} \in \mathbb{R}^{d \times 1 \times 1}$. 
% 
Note that $d$ indicates the dimension of each channel; $w$ and $h$ denote as the size of visual feature.
%
A batch of visual regions $\mathbf{V} = [\mathbf{v}_1,\mathbf{v}_2,\ldots,\mathbf{v}_k]$ and audio signals $\mathbf{A} = [\mathbf{a}_1,\mathbf{a}_2,\ldots,\mathbf{a}_k]$ with total $k$ pairs are the inputs.
% 
For each visual feature $\mathbf{v} = [\mathbf{v}(1),\mathbf{v}(2),\ldots,\mathbf{v}(w \times h)]$, it contains $w \times h$ patches.
% 
The model would be trained in total $n$ epochs.
%
For example, we illustrate our training framework with a audio-visual pair shown in Fig~\ref{fig:method}. 
% 
The input audio signal is transformed into frequency domain by short-time Fourier transform (STFT)~\cite{stft} and encoded as audio feature $\mathbf{a}$ by an audio network with global average pooling.
% 
As for visual feature $\mathbf{v}$, the input image is encoded by a visual network but without performing average pooling.  
% 

In Section~\ref{sec:av-learning}, we first introduce the initial audio-visual training scheme with contrastive learning as the paradigm for the following epochs. 
% 
We then further present our iterative learning strategy and proposed sampling techniques to learn discriminative audio-visual features. 
% 
How sound localization task can be achieved by audio-visual response will be demonstrated in section~\ref{sec:results}.


\subsection{Audio-Visual Representation Learning}
\label{sec:av-learning}

\Paragraph{Initial Contrastive Learning.} 
% how to train our baseline ... 
% \hyt{illustrate the learning scheme of the baseline.}
Natural audio-visual pairs from videos provide rich information to learn robust representation by optimizing an objective. 
% 
It maximizes correlation between sound and objects from the same pair (called positive pairs) and minimizes one between arbitrary audio and objects from different pairs (called negative pairs). 
% 
Such the property can be utilized as training objective function to learn audio-visual representation.
% 
The objective of contrastive loss can be expressed as follows: 
\begin{equation}
\begin{gathered}
\label{eq:nce_loss}
\mathcal{L}_{\text {contrast }}=-\log \frac{\exp \left(\phi(\overline{\mathbf{v}}_{i})^{\top} \cdot \overline{\mathbf{a}}_{i} / \tau_i\right)}{\sum_{j=0}^{k} \exp \left(\phi(\overline{\mathbf{v}}_{i})^{\top} \cdot \overline{\mathbf{a}}_{j} / \tau_i\right)}, \\
\forall i=\{1, \ldots,k\},
\end{gathered}
\end{equation}
where $\tau_i$ is a temperature parameter controlling the probability distribution from a softmax function. 
% 
$\phi$ and $\exp$ are average pooling function ($\phi(\mathbf{v}) \in \mathbb{R}^{d \times 1 \times 1}$) and exponential function. 
% 
$\overline{\mathbf{v}}$ and $\overline{\mathbf{a}}$ denote as $\ell_{2}$-normalized vectors.
% 
By \eqref{eq:nce_loss}, audio-visual representations are optimized at the initial stage (\eg the first five epochs).


\Paragraph{Iterative Contrastive Learning.}
% \hyt{1) baseline may use the features of incorrect region, 2) region annotation is not available, 3) describe proposed iterative scheme}
Although the audio-visual features can be learned by \eqref{eq:nce_loss}, it would include all visual patches containing either sounding or non-sounding regions. 
% 
The similarity between non-sounding objects and audio signal is maximized under this circumstance. 
% 
If sounding regions are known or accessible before performing contrastive learning, non-sounding regions would not be associated with the corresponding audio signal. 
% 
Nevertheless, there is no prior information about sounding regions in an unsupervised sound localization manner. 
% 


To this end, we consider potential sounding regions from the previous model into contrastive learning instead of directly performing average pooling on all visual patches. 
% 
To include potential sounding regions, we randomly sample visual patches which are highly related audio signals.
%
The stochastic sampling process can benefit representation learning by preventing models from overfitting training audio-visual pairs.
%
The visual features of sounding regions are described as follows:  
\begin{equation}
\begin{aligned}
\label{eq:pos_idx}
\mathbf{I}_{pos} &= idx(\overline{\mathbf{v}}^{\top} \cdot \overline{\mathbf{a}} > \delta_{v}), \\
\mathbf{v}^{+}&= \frac{1}{r}  \sum_{i=0}^{r} \mathbf{v}(\mathbf {I}_{pos}(i)),
\end{aligned}
\end{equation}
where $idx(.)$ returns the indexes of visual patches from given conditions in a random order, and $\delta_{v} \in [0,1]$ is a threshold for excluding non-sounding regions. 
% 
Note that the audio-visual features are extracted from the model from the previous epoch. 
% 
In~\eqref{eq:pos_idx}, $r$ is the number of sampled patches that is less than  $\mathbf{I}_{pos}$.
% 
If no patch is confident enough to be sounding regions, $\mathbf{v}^{+}$ would be replaced with $\phi(\mathbf{v})$.


\Paragraph{Intra-Frame Sampling.}
% \hyt{1) in the proposed iterative approach, we use psudo bbx as the positive example, 2) remaining region is not used, 3) we use it as additional negative example}]
% 
The key idea of contrastive learning is to model the relationship between all instances.
% 
It would be favorable to add additional instances as negative pairs. 
% 
However, directly sampling more negative pairs from other instances cannot benefit model training due to easy negative pairs which limit models to learn discriminative audio-visual features. 
% 
With aforementioned iterative contrastive learning scheme, we exploit the pseudo sounding regions as the positive examples. 
% 
Since some sounding objects are accessible from the paradigm model at previous epoch, the possible non-sounding regions can be further determined as well.
% 
Similarly, non-sounding regions can be obtained by:
\begin{equation}
\begin{aligned}
\label{eq:neg_idx}
\mathbf{I}_{neg} &= idx(\overline{\mathbf{v}}^{\top} \cdot \overline{\mathbf{a}} < \delta_{v}), \\
\mathbf{v}^{-}&= \frac{1}{r}  \sum_{i=0}^{r} \mathbf{v}(\mathbf {I}_{neg}(i)).
\end{aligned}
\end{equation}
Note that if no patch is lower the threshold, $\mathbf{v}^{-}$ would not be sampled.

\Paragraph{Inter-Frame Relation.}
Due to various objects in audio-visual pairs, audio-visual representations can be optimized by observing the correlation between audio and visual instances. %
We note that, the objects across videos may appear similar contents as shown in Fig~\ref{fig:teaser} (\eg trains appear in different pairs).
% 
However, the common contrastive learning schemes in an unsupervised manner would not associate between sounding objects and similar sound but in other pairs. 
% 

To this end, we propose a training strategy to associate sounding regions and audio even across pairs by observing relationship between all sound signals in the batch. 
% 
We can redefine the audio-visual pairs as follows:
\begin{equation}
\begin{aligned}
\label{eq:a_th}
y_{i,j}=\left\{\begin{array}{ll}
0, & \text { if } \overline{\mathbf{a}}_{i}^{\top} \cdot \overline{\mathbf{a}}_{j} < \delta_{a} \\
1, & \text { if } \overline{\mathbf{a}}_{i}^{\top} \cdot \overline{\mathbf{a}}_{j} \geq \delta_{a}\\
\end{array}\right. 
\forall i, j=\{1, \ldots,k\},
\end{aligned}
\end{equation}
where $\delta_{a} \in [0,1]$ is a threshold for adjusting the audio-visual pairs in the batch. With the redefined correlation and aforementioned sampling techniques, the training objective after initial contrastive learning is formulated as:
\begin{equation}
\label{eq:full}
\begin{aligned}
&\mathcal{L}_{\text {av-complex }}= \\ &-\log
\frac{\sum_{i,j=0}^{k} \exp ( (\overline{\mathbf{v}}_{i}^{+})^{\top} \cdot \overline{\mathbf{a}}_{j} / \tau_{itr}) y_{i,j}}
{\sum_{i,j=0}^{k} \exp ((\overline{\mathbf{v}}_{i}^{-})^{\top} \cdot \overline{\mathbf{a}}_{j} / \tau_{itr})
+ \exp ((\overline{\mathbf{v}}_{i}^{+})^{\top} \cdot \overline{\mathbf{a}}_{j} / \tau_{itr})
}.
\end{aligned}
\end{equation}
Note that we optimize our framework by~\eqref{eq:nce_loss} at initial stage. Otherwise, the model is trained with~\eqref{eq:full}.


% \subsection{Sounding Object Localization}
% \label{sec:localization}
 

==> backup/4_results_bk.tex <==

% \input{table/stoa.tex}

\section{Experimental Results}
\label{sec:results}

%\subsection{Datasets}
%\label{sec:dataset}
\Paragraph{Datasets.} The \textbf{SoundNet-Flickr}~\cite{av_nips16_soundnet} dataset consists of more than two million video sequences.
% 
We use the $5$-seconds audio clip and corresponding image, \ie video frame extracted from the center of the $5$-seconds interval, to form the input pair for the proposed framework.
% 
Note that we do not rely on any annotation (\eg bounding boxes) for the training.
%
In all experiments, we perform the training using the subset of the SoundNet-Flickr dataset constructed by Qian~\etal~\cite{av_eccv20_mms_loc} that contains $10$k audio-visual pairs.
%
Following the protocol in~\cite{av_eccv20_mms_loc,av_cvpr18_lls,av_tpami20_lls}, we conduct the evaluation using the testing set o the SoundNet-Flickr dataset that consists of $250$ audio-visual pairs with bounding box annotations.
%
%As for quantitative evaluation, Senocak~\etal~\cite{av_cvpr18_lls,av_tpami20_lls} provide bounding boxes of sounding regions for the subset of SoundNet-Flickr, which contains 5k annotations.
% 
%In our experiment, we train with 10k pairs (no supervision) in a random sample subset\footnote{github.com/shvdiwnkozbw/Multi-Source-Sound-Localization} of SoundNet-Flickr, which are the \yb{exact} same pairs as~\cite{av_eccv20_mms_loc}.
% 
%To fairly compare with the methods, the evaluation is performed in test set of SoundNet-Flickr~\cite{av_cvpr18_lls,av_tpami20_lls} containing 250 audio-visual pairs with bounding box annotations. 
% 
%\yb{The aforementioned settings are following the ones in~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_mms_loc}}.

\input{table/stoa}
\Paragraph{Implementation Details.} We implement the proposed method using Pytorch~\cite{pytorch}, and conduct the training as well as evalution on a single NVIDIA GTX 1080 Ti GPU with $12$ GB memory.
%
Specifically, we use the ResNet-18~\cite{resnet} model for both the visual and audio feature extractors.
%
Note that we adopt the strategy in~\cite{av_eccv20_mms_loc} that uses the visual feature extractor pre-trained on the ImageNet~\cite{ImageNet} dataset.
%
As for the data pre-processing, the raw 5-seconds audio clips are re-sampled at $22.05$ kHZ, then transformed into the log-mel spectrograms~(LMS) using $64$ frequency bins and the window of size $40$ ms for every $20$ ms.
%
The images are re-sized to the resolution of $256\times 256$.
%
For fair comparisons, we adopt the batch size of $96$ which is used in~\cite{av_eccv20_mms_loc} for all the experiments since a larger batch size may benefit our contrastive learning approach.
%
More implementation details are presented in the supplementary material.
%
We will release the source code stimulate future research.

%\Paragraph{Sound Localization.}
\ybc{main reason for initial model beats STOAs}
We first compute the response map $\mathbf{R}$ using Eq.~\eqref{eq:cos}.
%
Then we recover the resolution of the response map $\mathbf{R}$ from $w\times h$ to original image resolution $W \times H$ using bilinar up-sampling and min-max normalization on each instance:
\begin{equation}
\label{eq:normalization}
\mathbf{R} = \frac{\mathbf{R}_i -\min(\mathbf{R}_i)}{\max(\mathbf{R}_i) - \min(\mathbf{R}_i)},
\quad i=1\sim k.
\end{equation}
%
Finally, we the re-scale the values in the response map to the be in the range of $[0, 1]$.


%With audio and visual representation, it is possible to recognize sounding regions by calculating the response between visual patches and audio signal by~\eqnref{cos}.
% 
% We calculate the response with cosine similarity:
% \begin{equation}
% \label{eq:cos}
% \mathbf{C} = \overline{\mathbf{v}}^{\top} \cdot \overline{\mathbf{a}},
% \end{equation}
% where $\mathbf{C} \in \mathbb{R}^{1 \times w \times h}$ is the response maps for visual patches. 
%To correspond the size of image input, we perform bilinear up-sampling on response maps 

\Paragraph{Evaluation Metrics.}
\hyt{cannot understand this section, refer the previous paper and make it more clear}
%\Paragraph{From Bounding Box to Score Map.}
Following~\cite{av_cvpr18_lls,av_tpami20_lls,av_eccv20_mms_loc,av_cvpr19_deep_cluster,av_arxiv_curricumlum_av_clutser}, 
The bounding box annotations in coordinate form are transformed into binary maps.
% 
Note that there are multiple $N$ bounding boxes for each image (\eg $\mathbf{b}_1$ is one of the boxes).
% 
To be more specific, the patches of non-sounding/sounding regions are labeled as 0 and 1 respectively. 
% 
The representative score map $\mathbf{g}$ can be described as follows:
\begin{equation}
\label{eq:loc_gt}
\begin{aligned}
\mathbf{g}=\min \left(\frac{\sum_{i=1}^{N} \mathbf{b}_{i}}{\# \text { consensus }}, 1\right),
\end{aligned}
\end{equation}
where \#consensus is a minimum number of agreement. For example, the minimum number of people considering whether a pixel makes sounds or not. 
% 
We set \#consensus $=2$, which is suggested by~\cite{av_cvpr18_lls,av_tpami20_lls}.
% 

With ground truth score map $\mathbf{g}$, 
\textbf{consensus intersection over union (cIoU)} and \textbf{area under curve (AUC)} are utilized for measuring the quality of predicted sound localization results. 

\Paragraph{Baseline methods.}
We compare our method train with the $10$k audio-visual with the following weakly-supervised or unsupervised approaches: \hyt{do not introduce how these methods work, focus on 1) what/how manay training pairs used 2) do they use any assumption or event label}
%To evaluate the quality of our predicted sound localization, we compare our method (10K audio-visual pairs) with the following state-of-the-arts methods in a weakly supervised or unsupervised manner:
\begin{compactitem}
\item\textbf{Attention 10K~\cite{av_cvpr18_lls,av_tpami20_lls}:} The model leverages audio-visual co-attention mechanism during representation learning.

\item \textbf{DMC AudioSet~\cite{av_cvpr19_deep_cluster}:} Audio-visual clusters are utilized to minimize the distance of center audio and visual features. It is trained on AudioSet-Balanced-Train~\cite{Audioset} with 20K samples and test on SoundNet-Flick dataset.

\item \textbf{CAVL AudioSet~\cite{av_arxiv_curricumlum_av_clutser}:} 
The audio-visual cluster based method with a curriculum learning strategy to handle with number of sounding source. The training and testing scenario are the same as DMC~\cite{av_cvpr19_deep_cluster}. 
\item \textbf{MSSL 10K/20K~\cite{av_eccv20_mms_loc}:} As a state-of-the-art method for sound localization, it utilizes audio/visual event labels and CAM~\cite{cvpr16_CAM} to find sounding regions with 10K/20K training samples.

\end{compactitem}


\input{figure/cIoU_curve}
\input{figure/vis.tex}
\subsection{Quantitative Results}
% 
\tabref{stoa} shows the quantitative comparisons on the SoundNet-Flickr dataset.
% 
The proposed method performs favorably against the baseline approaches.
%
We note that different from the proposed method, the DMC, CAVL, MSSL schemes require prior assumption \hyt{be specific, what assumption}.
%
Furthermore, our model trained with $10$k audio-visual pairs show more accurate sound localization results than the MSSL-$20$k approach that uses more (\ie $20$k) audio-visual pairs for the training.
%
In addition to the cIoU\@$0.5$ metric, we present the cIoU scores calculated with various thresholds \figref{curve}.
%
Our method reports favorable cIoU scores under all thresholds, suggesting the effectiveness of the proposed iterative contrastive learning algorithm.


\input{figure/vis_abs.tex}
\input{table/ablation}
\subsection{Qualitative evaluation}
The visualization results are shown in Fig.~\ref{fig:vis} on image-sound pairs selected from the SoundNet-Flicker dataset. 
% 
From this figure, we see that our method presents more accurate sound localization results.
% 
The example in the top row is particularly challenging. Since trains usually run on the rail, models for unsupervised sound localization would jointly associate rails and trains with train sounds. 
% 
As for MSSL, due to the guide of audio/visual event labels, it can reduce influences from the noise background.
% 
It is worth noting that, no prior assumption is available our during model training. Instead, DMC, CAVL and MSSL require pre-defined number of sound source or audio/visual event labels. 
% 
Thus, these results support the use of our training strategy for discovering the sounding objects in a scene.


\input{figure/vis_inter}
\input{figure/vis_itr}
\subsection{Ablation Study}
\Paragraph{Localization and Normalization.}
Since we adopt state-of-the-art model~\cite{av_eccv20_mms_loc} with different localization and visualization technique to localize sound,
the investigation of these techniques are desirable.
% 
The brief summarization of MSSL~\cite{av_eccv20_mms_loc} is illustrated as follows:
% 
MSSL~\cite{av_eccv20_mms_loc} a two-stage sound localization model trained with extra audio-visual event labels.
% 
The event classifiers and audio-visual correspondence are utilized during the first stage.
% 
The additional label-guide contrastive learning is applied at the second stage.
% 
When the model can understanding vision and audio signals,
the sound localization results are achieved by CAM with normalizing the maximum value to one. 
% 
Note that such details in our model are described in~\eqnref{cos} and~\eqnref{normalization}.

In \tabref{ablation}, the top block indicates the results with original MSSL setting. 
% 
We can see that the performance is degraded significantly since CAM requires labels to find discriminative regions.
% 
As for the second top block, audio-visual correlation~\eqnref{cos} is utilized to find sounding regions instead of CAM.
% 
The first stage of MSSL with~\eqnref{cos} can achieve favorable performance compared with the methods, whose localization results are calculated by CAM.
% 
For the third block, we further apply minmax normalization mechanism~\eqnref{normalization}, where the results within an instance are normalized to values from zero to one. 
% 
The minmax normalization~\eqnref{normalization} can strengthen the localization results in cIoU metric at 0.5 threshold, which indicates the improvement by~\eqnref{normalization} only at certain threshold.
% 
For the bottom block, we compares and verifies the contribution of every components in our method, where Itr, Intra, and Inter denote iterative contrastive learning, intra-frame sampling, and inter-frame relation respectively described in~\secref{av-learning}. 
% 
Check mark indicates methods which are utilized.
% 
Note that the initial contrastive learning~\eqnref{nce_loss} is able to achieve favorable performance against MSSL. 
% 

Furthermore, the localization results with each module in our model are presented in~\figref{vis_abs}. 
% 
We can see that our training strategy is able to effectively alleviate the noise of non-sounding regions. 
% 
It is clear that iterative contrastive learning can provide more accurate results than initial one, and the results from our proposed method are correctly localized on sounding regions compared with only iterative contrastive learning (without intra-frame sampling and inter-frame relation).
% 
Note that intra-frame sampling and inter-frame relation are based on iterative contrastive learning.

\Paragraph{Paradigm from Previous Epoch.}
Since our model is based the results from the model at previous epoch as pseudo-annotation for current model learning, the localization results at different epoch play a critical factor of performance.
% 
To this end, we investigate the localization results at different epochs in~\figref{vis_itr}.
% 
In~\figref{vis_itr}, the localization results are gradually accurate to sounding regions, which indicates the model from previous epoch can provide favorable guide for the current model learning.


\Paragraph{From Sound to Associate Objects.}
As discussed earlier, since inter-frame relation is based on the correlation between audio signals within a batch, the visualization can explain the justification of the model design.
% 
That is, given an audio-visual pair, we would like to explore the related sounding objects by audio signals.
% 
In~\figref{vis_inter}, the first and fifth column with reference caption is the anchor images. The corresponding audio signals are utilized to measure the correlation of all testing data.
% 
We find the top three similar sound and present the corresponding images in the following columns.
% 
Our assumption that sounding objects are related if their sounds are similar is verified with the cases in~\figref{vis_inter}, which alleviates typical contrastive learning methods from differentiating the sounding object and related audio signals.
% 











==> backup/abstract_bk.tex <==
\begin{abstract}
%
Human beings perform various tasks by jointly perceiving multisensory signals.
%
However, it is time-consuming and labor-intensive to annotate the correlations of signals from multiple sensors (modalities), thus making it difficult supervise a machine to learn such tasks.
%
In this work, we focus on the sound localization task, which relies on the mutual understanding of visual and audio cues to associate sounds with corresponding objects in the visual scene.
%
We propose an iterative contrastive learning framework that requires no data annotation. 
%
Starting from simple contrastive learning, the proposed training method iteratively takes the localization results predicted in the previous epoch as pseudo-annotations of sounding and non-sounding regions, and learns the correlation between visual and audio signals within instances as well as the correlation between audio signals across instances. 
%
The training method encourages localization of sounding regions and reduces association between non-sounding objects with audio sources. 
%By exploiting the localization results from previous epoch, our training strategy can utilize (non-)sounding regions to learn robust audio-visual features to achieve accurate localization results.
%
%Furthermore, we observe the correlation between audio signals across instances, which prevents non-sounding  objects associated with audio source.
%
Quantitative and qualitative experimental results demonstrate that the proposed self-supervised framework performs favorably against existing unsupervised and weakly-supervised methods for sound localization.
%Experiments on the benchmark dataset validate the effectiveness of our proposed framework in an unsupervised scenarios, with ablation studies and visualization further support the use of our model for sound localization.


% \keywords{Audio spatialization, self-supervised learning, deep learning}


\end{abstract}  

==> figure/att_func.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.95\linewidth]{figure/images/att.png}
 	%\vspace{-2mm}
     \caption{\textbf{Learning co-attention of audio-visual features as a cue for binaural audio prediction.} For each audio component (out of $u \times t$) in the spectorgram, we perform correlation between it and the observe visual feature, which identifies the corresponding spatial region(s) of interest. With left and right weighting functions applied, the left-right audio-visual relationship can be derived and guide the learning of left-right audio difference in our framework.}
	\label{fig:att_func}
\end{figure*}

==> figure/semi.tex <==
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[h]{0.48\linewidth}
    \includegraphics[width=\linewidth]{figure/images/semi_env.pdf}
    \caption{Envelope (ENV) Distance}
    \label{fig:semi_env}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.48\linewidth}
    \includegraphics[width=\linewidth]{figure/images/semi_STFT.pdf}
    \caption{STFT Distance}
    \label{fig:semi_stft}
    \end{subfigure}%
 	%\vspace{-2mm}
     \caption{Performance comparisons in terms of ENV and STFT on FAIR-PLAY using different amount of video data with ground truth binaural audio for training. Note that the horizontal axes in both figures reflects the percentage of data with ground truth audio utilized. It can be seen that our model achieved comparable results as other fully supervised models did, while only about 60\% of labeled data were used when training our model.}
	\vspace{-5mm}
	\label{fig:semi}
\end{figure*}

==> setup/graphicspath.tex <==
\graphicspath{{figure}, {images}, {example}}


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}


==> table/frame.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering

\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|ccccc}
\begin{tabular}[c]{@{}c@{}}Partition \\ Ratio\end{tabular} & $\frac{1}{8}$    & $\frac{1}{4}$    & $\frac{1}{2}$   & $\frac{2}{3}$   & $\frac{3}{4}$    \\ \hline \hline
ENV                                                        & 0.1011 & 0.0995 & 0.0982         & \textbf{0.0973} & 0.0997 \\
STFT                                                       & 1.082  & 1.054  & \textbf{0.992} & 0.998           & 1.010 
\end{tabular}%
}
\vspace{2mm}
\caption{Comparisons of binaural audio prediction in different partition ratios of visual frames in 50\% ground truth binaural audio usage which better expresses the influence of $\mathcal{L}_{tri}$. The spatial awareness correlation loss $\mathcal{L}_{tri}$ jointly considers in-frame negative samples. The in-frame negative samples rely on splitting a video frame into left and right. The first row shows the ratio of partition for a video frame. The numbers in bold indicate the best results.}
\label{tab:frame}
\end{table}

==> table/stoa2.tex <==


\begin{table}[t]
    \caption{\textbf{Quantitative results of sound localization.} \yb{We conduct the experiments on the MUSIC-Synthetic~\cite{av_nips20_loc} dataset containing multiple sound sources of instruments, and evaluate the cIoU@$0.3$ and AUC scores. The best performance is reported in \textbf{bold}. }}
    \label{tab:stoa_music}
    \centering
    \normalsize
    \begin{tabular}{l cc}
        \toprule\
         & cIoU@0.3 $\uparrow$ & AUC $\uparrow$\\
        \midrule
        Attention ~\cite{av_cvpr18_lls} & $6.9$ & $14.2$ \\
        DMC ~\cite{av_cvpr19_deep_cluster} & $6.6$ & $15.3$ \\
        MSSL ~\cite{av_eccv20_mms_loc} & $4.3$ & $12.1$ \\
        DSOL ~\cite{av_nips20_loc} & $15.4$ & $17.0$  \\
        \midrule
        Ours & $\mathbf{19.8}$ & $\mathbf{22.7}$ \\
        \bottomrule
    \end{tabular}
    \vspace{0mm}
\end{table}





% \begin{comment}
% \begin{table}[t]
% \centering
% \resizebox{0.4\textwidth}{!}{%
% \begin{tabular}{c|l|c|l|cl}
% \multicolumn{2}{c|}{Method}        & \multicolumn{2}{c|}{cIoU@0.5}      & \multicolumn{2}{c}{AUC}           \\ \hline
% \multicolumn{2}{c|}{Random}        & \multicolumn{2}{c|}{7.2}           & \multicolumn{2}{c}{30.7}          \\
% \multicolumn{2}{c|}{Attention 10K~\cite{cvpr18_lls}} & \multicolumn{2}{c|}{43.6}          & \multicolumn{2}{c}{44.9}          \\
% \multicolumn{2}{c|}{DMC AudioSet}  & \multicolumn{2}{c|}{41.6}          & \multicolumn{2}{c}{45.2}          \\
% \multicolumn{2}{c|}{CAVL AudioSet} & \multicolumn{2}{c|}{50.0}          & \multicolumn{2}{c}{49.2}          \\
% \multicolumn{2}{c|}{MSSL 10K}      & \multicolumn{2}{c|}{52.2}          & \multicolumn{2}{c}{49.6}          \\
% \multicolumn{2}{c|}{MSSL 20K}      & \multicolumn{2}{c|}{53.8}          & \multicolumn{2}{c}{50.6}          \\ \hline \hline
% \multicolumn{2}{c|}{Ours 10K}      & \multicolumn{2}{c|}{\textbf{75.9}} & \multicolumn{2}{c}{\textbf{60.3}}
% \end{tabular}
% }
% \caption{Performance comparisons of sound localization in terms of cIoU and AUC. Note that the numbers in bold indicate the best results.
% }
% \label{tab:stoa}
% \end{table}
% \end{comment}
